Triple Sparsification of Graph Convolutional Networks without Sacrificing the Accuracy

Graph Neural Networks (GNNs) are widely used to perform different machine learning tasks on graphs. As the size of the graphs grows, and the GNNs get deeper, training and inference time become costly in addition to the memory requirement. Thus, without sacrificing accuracy, graph sparsification, or model compression becomes a viable approach for graph learning tasks. A few existing techniques only study the sparsification of graphs and GNN models. In this paper, we develop a SparseGCN pipeline to study all possible sparsification in GNN. We provide a theoretical analysis and empirically show that it can add up to 11.6\% additional sparsity to the embedding matrix without sacrificing the accuracy of the commonly used benchmark graph datasets.

==> background.tex <==
\section{Background}
\subsection{Notations}
Let $G(V, E)$ be a directed graph, where $V=\{v_1, \ldots v_n\}$ is the set of vertices and $E=\{e_1, \ldots, e_m\}$ is the set of edges such that $|V|=n$, and $|E|=m$. Here, each $e_i = (v_a, v_b) \in E$ means that there is an edge between vertex $v_a$ and vertex $v_b$. Also assume that $\vect{X}\in \mathbb{R}^{n\times d}$ represents the $d$-dimensional input features of $n$ vertices. We represent the adjacency matrix of $G$ by $\vect{A}$, where $\vect{A}_{ij}=1$ if $(v_i, v_j)\in E$, otherwise $\vect{A}_{ij}=0$. The computation at the $l$-th layer of GCN \cite{kipf2016semi} is:
\begin{equation}
\label{eqn:gcn}
    \vect{H}^{l} = \sigma(\vect{\hat{A}}\vect{H}^{l-1}\vect{W}^{l-1})
\end{equation}
where, $\vect{W}$ is the neural network weight matrix, $\sigma$ is the activation function and $\vect{H}$ is the hidden representation of corresponding convolutional layer such that $\vect{H}^0 = \vect{X}$. In Eqn. \ref{eqn:gcn}, $\vect{\hat{A}}$ is the renormalized graph Laplacian matrix such that $\vect{\hat{A}}=\vect{\tilde{D}}^{-\frac{1}{2}}\vect{\tilde{A}}\vect{\tilde{D}}^{\frac{1}{2}}$, $\vect{\tilde{A}} = \vect{I} + \vect{A}$, where $\vect{I}$ is the identity matrix, and $\tilde{D}_{ii} = \sum_{j}\tilde{A}_{ij}$. Let us consider that $\vect{H}^{L}$ is the hidden representation of the last layer of GCN and $\vect{Y}$ represents the one-hot encoded node labels for the vertices $V$, then we can define the semi-supervised loss function for the node classification problem as follows:
\begin{equation}
    \label{eqn:loss}
    \mathcal{L} = -\frac{1}{|c_i|}\sum_{i \in n} Y_i\log H^{L}_i
\end{equation}
where, $c_i$ is the number of labels for vertex id $i$, and $\mathcal{L}$ is the negative log-likelihood loss function. 

Let us assume that $m^l_w$ and $m^l_h$ represent two differential binary masks of weights and embedding, respectively on the $l$-th layer of the GCN model. If we reset (assign 0's) some non-zero entries of $m^l_w$, then, $m^l_w\odot \vect{W}^l$ would necessarily sparsify the weight matrix in the $l$-th layer, where $\odot$ is an element-wise product operator. Similarly, $m^l_h\odot \vect{H}^l$ would sparsify the embedding matrix in the $l$-th layer.

\subsection{Related Work}

\textbf{Graph Neural Networks.} In recent years, Graph Neural Networks (GNN) have become popular to solve graph learning tasks such as node classification, link prediction, and graph classification. The very first Graph Convolutional Networks (GCN) is a pioneering work in this research area that focuses on learning representation from neighbors in a semi-supervised way using summation as an aggregation function \cite{kipf2016semi}. GraphSAGE method advances the field by introducing some other aggregation functions \cite{hamilton2017inductive}. Though these earlier works have advanced the graph learning tasks \cite{kipf2016semi, hamilton2017inductive, velivckovic2017graph,xu2018powerful}, they are limited by some bottlenecks such as over-smoothing problem or neighborhood explosion problem \cite{alon2020bottleneck,oono2019graph}. Some methods have also been proposed to address such issues in the literature \cite{chiang2019cluster}. Nonetheless, efficient training of large graphs is still a challenging task due to the size of different matrices in Eqn. \ref{eqn:gcn}. Thus researchers also focus on optimized resource usages in GNN by sampling sub-graphs or partitioning the original graphs \cite{li2021training}.

\textbf{Sparsifications of Neural Networks.}
Sparsification is being studied well by the deep learning community. The main focus of the sparsity of Convolutional Neural Networks (CNN) is
on weight parameters. It helps compress the learned model that results in a faster inference time. An earlier study by Song et al. showed that the neural network model could be compressed up to 9 fold without losing accuracy \cite{han2015learning}. After that, they improved the compression for better memory utilization by employing quantization and Huffman coding \cite{han2015deep}. Forrest et al. also studied the problem and achieved a compression factor of 50 \cite{iandola2016squeezenet}. Hao et al. studied the pruning of convolutional filters and feature maps which also improves the inference time \cite{li2016pruning}. Siddhant et al. proposed Top-KAST to train a sparse model~\cite{jayakumar2021top}. There are other studies in the literature for neural network sparsifications techniques to improve the model compression and achieve better inference time \cite{frankle2018lottery,liu2021selfish,han2016eie}. There are several survey papers for deep convolutional neural networks that summarize the sparsification or acceleration strategies \cite{hoefler2021sparsity,gale2019state,abadal2021computing}. Overall, the sparsification of neural networks in the image domain is a heavily studied problem.
\begin{table}[!htb]
\centering
\caption{Papers discussing pruning strategy of a GNN.}
\vspace{-0.35cm}
\arrayrulecolor{black}
\label{tab:papers}
\begin{tabular}{c|p{1.2cm}p{1.3cm}p{1.2cm}} 
\hline
Paper(s) & Prune $\vect{\hat{A}}$? & Prune $\vect{W}$? & Prune $\vect{H}$? \\ \hline
SGCN~\cite{li2020sgcn}, FastGCN~\cite{chen2018fastgcn}    &        \textbf{\ding{52}}                                                  &                               \textbf{\ding{55}}                              &     \textbf{\ding{55}}                                                             \\ 

ULTH~\cite{chen2021unified}, GEBT~\cite{you2021gebt}     &\textbf{\ding{52}}                                                          &                               \textbf{\ding{52}}                            &                               \textbf{\ding{55}}                                  \\ 

SparseGCN (Ours)     & \textbf{\ding{52}}  & \textbf{\ding{52}}  &  \textbf{\ding{52}}                                                                                                                                          \\
\hline
\end{tabular}
\arrayrulecolor{black}
\end{table}
\vspace{-0.15cm}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/workflow.pdf}
    \vspace{-0.25cm}
    \caption{Example of (a) graph sparsification by removing edges (dotted lines), (b) embedding matrix sparsification by assigning zero, and (c) weight sparsification by removing edges in the GCN model. (d) A workflow of our sparse training procedure. An input graph with node features is fed to the GCN model. It is trained for $n$ epochs and records the test accuracy. After that, a sparse routine introduces sparsity in adjacency, embedding, and weight matrice, and then the model is trained again. The sparsification and re-training steps continue until we achieve an optimal level of sparsity without sacrificing test accuracy.}
    \vspace{-0.25cm}
    \label{fig:workflow}
\end{figure*}

\textbf{Sparsifications in Graph Neural Networks.} Dense hardware can speed up the training~\cite{balog2019fast} of GNNs but as the size of the graph grows, the limitations of memory requirement and computation time become obvious. In GNNs, three matrices are involved (see Eqn. \ref{eqn:gcn}) that can be sparsified jointly or separately. In the literature, the sparsification of GNNs has been tackled by researchers considering two directions: (i) input graph or adjacency matrix sparsification, and (ii) model weight sparsification. The former has been studied much in the GNN literature; however, the latter has not been explored much. For example, FastGCN \cite{chen2018fastgcn} and GraphSAINT \cite{zeng2019graphsaint} focus on the sampling of subgraphs/edges/nodes from the input graphs. This approach necessarily prunes the adjacency matrix that results in a faster training time. Noticeably, the $\tilde{A}$ in Eqn. \ref{eqn:gcn} is already a sparse matrix for graph. Further sparsification can show high sensitivity by reducing the accuracy for scale-free networks. There are a handful of studies in the literature that discuss such sparsifications of graphs \cite{ye2021sparse,li2020sgcn}. However, we observe a few studies in the literature for GNN model compression. In recent years, Unified lottery Ticket Hypothesis (ULTH) \cite{chen2021unified} and early-bird ticket \cite{you2021gebt} are the two noticeable works for both graph and model weight sparsifications in GNNs. However, the embedding matrix sparsification has not been explored previously except random \emph{dropout} for regularization. We summarize the pruning or sparsification related papers of GNN in Table \ref{tab:papers}. If we revisit Eqn. \ref{eqn:gcn}, we observe that all three matrices of GCN can be sparsified which has not been studied in the literature to the best of our knowledge. Thus, we study the fully sparse GCN by analyzing the sensitivity of different sparse matrices in Eqn. \ref{eqn:gcn}.





==> methods.tex <==

\section{Methods}
We use GCN as a representative GNN method to induce sparsity in different matrices. Firstly, we train the GCN model with original matrices  to obtain the baseline accuracy. Then, we retrain the model after sparsifying various networks. We describe different steps of SparseGCN as follows.

\begin{algorithm}[!htb]
\caption{SparseGCN Training for Node Classification}\label{algo:training}
\begin{flushleft}
\textbf{Input:} $\vect{A}$: adjacency matrix of an input graph, $\vect{X}$: input feature, $\vect{W}^1, \vect{W}^2:$ initial weights of GCN, initial masks $m^1_h, m^2_h$: embedding masks, $m^1_w, m^2_w$: weight masks, $a$: sparsity for adjacent matrix, $w$: sparsity for weight matrices, $h$: sparsity for embedding matrices.\\
\textbf{Output:} the pruned adjacency matrix $\vect{A}$, network weight $\vect{W}\odot m_w$, embedding $\vect{H}\odot m_h$, and the optimal sparsity levels. 
\end{flushleft}
\begin{algorithmic}[1]
%\Procedure{SparseGCN}{}
    \For{$i\leftarrow 1 \ldots max\_epoch$}
        \State Forward propagation using Eqn. \ref{eqn:gcn} and update $\vect{H}$
        \State Backward propagation with loss of Eqn. \ref{eqn:loss} and update $\vect{W}$
        \State Update the learning step
    \EndFor
    \State Sparsify $a\%$ non-zero entries of adjacency matrix based on the weight of $\vect{\hat{A}}$
    \State Sparsify $w\%$ non-zero entries of $m^l_w$ based on $\vect{W}^l$ and obtain $\vect{W}^l = m^l_w\odot \vect{W}^l$
    \State Sparsify $h\%$ non-zero entries of $m^l_h$ based on $\vect{H}^l$ and obtain $\vect{H}^l = m^l_h\odot \vect{H}^l$
\State \Return sparse matrices $\vect{\hat{A}}, \vect{W}$, and $\vect{H}$
%\EndProcedure
\end{algorithmic}
\label{algo:training}
\end{algorithm}

\subsection{Algorithmic Workflow}
Our training protocol, after adding sparsity to the model, is similar to most of the methods in the literature \cite{you2021gebt,chen2021unified,li2020sgcn}. We followed the protocol  used in the unified lottery ticket hypothesis paper~\cite{chen2021unified}. 
% We show the schematic diagrams for sparsity in the graph, embedding, and weight in Figs. \ref{fig:workflow}(a)-(c). We also show the workflow in Fig. \ref{fig:workflow}(d). 

\textbf{Graph Sparsification.} 
To add sparsity to the graph or adjacency matrix, we remove a subset of edges from the graph. In Fig. \ref{fig:workflow}(a), we show the removed edges by dotted lines. Since the sparsified graph is used in all layers, we do not create additional masks for different layers. In this step, we remove $a\%$ edges from the weighted adjacency matrix $\vect{\hat{A}}$ using a chosen sparsification technique.

\textbf{Embedding Sparsification.} Unlike previous work, we also sparsify the embedding matrix as shown in Fig. \ref{fig:workflow}(b). In the schematic diagram, we assume that the entries in the embedding matrix are within the range of 0 to 1. To sparsify it, we select $h\%$ non-zero entries and mask them out by setting them to 0. We perform this sparsification step with a  Boolean mask $m^l_h$ and then masking entries from the embedding matrix with the mask $m^l_h\odot \vect{H}^l$. This operation also ensures that masked values in $\vect{H}^l$ are not updated in the current gradient descent iteration. %  by the gradient update procedure.

\textbf{Weight Sparsification.} Similar to previous studies \cite{chen2021unified,you2021gebt}, we also sparsify model weights of GCN in different layers as shown in Fig. \ref{fig:workflow}(c). We mask out a fraction of non-zero entries from the weight matrix using the operation $m^l_w\odot \vect{W}^l$. Similar to the embedding sparsification, this operation ensures that masked values in $\vect{W}^l$ are not updated in the current iteration.

In the workflow, as shown in Fig. \ref{fig:workflow}(d), we train the GCN model for the input graph with associated node features to obtain the baseline accuracy for the node classification problem. After that, we sparsify the graph, embedding matrix, and weight matrix using a sparsification technique described in Section \ref{sec:sparsification}. Then, we re-train the model with sparsified matrices and compare the accuracy level. If it is similar to the baseline accuracy, we sparsify the sparse matrices again and re-train the model. We continue this process until the accuracy level drops compared to the baseline. Finally, we report the highest sparsity level for which the sparsed model can retain the baseline accuracy. The training procedure of a 2-layered SparseGCN is shown in Algorithm \ref{algo:training}. We train the model $max\_epoch$ number of iterations, introduce a certain level of sparsity to the matrices, and return the sparse matrices.

\subsection{Sparsification Techniques}
\label{sec:sparsification}
\;\;\;\;\textbf{Random.} This is a naive and straightforward approach for the sparsification of any matrices in Eqn. \ref{eqn:gcn}. We pick $p\%$ entries from the non-zero elements of the matrices and mask them out by assigning zero to them. It can be a baseline approach that has also been used in the earlier studies \cite{chen2021unified}. Notably, this approach is similar to the \emph{dropout} of neural networks for regularization \cite{hinton2012improving}.

\textbf{Sorting-based.} This approach focuses more on global sparsification. At first, we sort all the non-zero entries of the matrices based on the absolute values. Then, we pick the smaller $p\%$ entries and mask them out by assigning zero. The rationale for this technique is that we can remove more insignificant entries globally which will have less computational effect compared to the local sparsification. Thus, we will be able to remove less sensible entries more retaining a similar level of accuracy. This technique has also been used by earlier studies of DNNs~\cite{chen2020lottery,renda2020comparing,chen2021unified}.

\textbf{Top-$k$.} We use this technique in GCN sparsification for the first time where each row of the matrix is sorted based on the absolute value of the non-zero entries. Then, we select the smaller $k$ entries from each row and mask them out by assigning zero. This technique focuses more on local sparsification. The intuition behind this approach is that the absolute smaller non-zero entries contribute less to the matrix multiplication. Thus, removing a few of them will not change the computations which are expected to retain a similar level of accuracy.
\vspace{-0.35cm}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.32\linewidth,height=2.0cm]{figures/weight_before.pdf}
    \includegraphics[width=0.32\linewidth,height=2.0cm]{figures/weight_clipped.pdf}
    \includegraphics[width=0.32\linewidth,height=2.0cm]{figures/weight_after.pdf}
    \vspace{-0.25cm}
    \caption{Left plot shows the distribution of values in the weight matrix of the first convolutional layer of GCN. Middle plot shows the distribution of pruned weight. Right plot shows that the retrained model regains the similar distribution but the mean and standard deviation can differ.}
    \vspace{-0.35cm}
    \label{fig:sensitive_prune}
\end{figure}

\textbf{Sensitivity-based.} Similar to Top-$k$, we also explore this technique in GCN sparsification for the first time. In Fig. \ref{fig:sensitive_prune} (left plot), we show the distribution of values of weight matrix in the first layer of GCN before pruning. It follows a normal distribution which is similar to the CNN \cite{han2015learning}. Thus, we could use the standard deviation of the distribution to prune some values. In Fig. \ref{fig:sensitive_prune} (middle plot), we see that the pruned weights are mostly around the 0 means. In the right plot, we show that the re-trained model achieves a similar normal distribution again after pruning but with a different mean and standard deviation. We can define the sensitive threshold $\theta = \lambda\sigma$, where $\sigma$ is the standard deviation, and $\lambda$ is a scaling factor. Then, we can prune non-zero entries from the weight matrix whose absolute value is less than $\theta$.

\subsection{Theoretical Analysis}
The number of non-zero entries in $\vect{\hat{A}}$, $\vect{W}^l$, and $\vect{H}^l$ matrices mostly depend on the input graph and the embedding dimension. 
In our analysis, we focus on the computation in the $l$th layer of a GNN, but the obtained bounds are applicable to other layers without loss of generality. 
We assume that the adjacency matrix $\vect{\hat{A}}$ containing $m$ edges is stored in the compressed sparse row (CSR) format so that the memory requirement is $O(m)$, and the number of Floating-point Operations (FLOPs) in sparse-dense matrix multiplication meets its lower bound~\cite{koanantakool2016communication}.
% \checkme{
% To simplify the analysis, we focus on a specific layer of the GCN in such a way that the computation of other layers can easily be inferred. Notice that the adjacency matrix $\vect{\hat{A}}$ with $m$ edges is often represented as a compressed sparse row format  \cite{saad2003iterative} for the optimal number of Floating-point Operations (FLOPs) in sparse-dense matrix multiplication~\cite{koanantakool2016communication}}. 
Suppose, the dimensions of $\vect{H}^l$, and $\vect{W}^l$ matrices in the $l$-th convolutional layer of GCN are $n\times d$, and $d\times f$, respectively. Then, we can deduce the following bounds.

\begin{lemma}
\label{lem:upper} The total number of MAC operations on the $l$-th layer is $(fm+dfn-fn)$, where $d > f$.
\end{lemma}
\begin{proof}
For $d > f$, the right ordered multiplications (i.e., $\vect{\hat{A}}(\vect{H}^l\vect{W}^l)$) in Eqn. \ref{eqn:gcn} would cost less computations than the left order (i.e., $(\vect{\hat{A}}\vect{H}^l)\vect{W}^l$). The total number of FLOPs for $\vect{T} = \vect{H}^l\vect{W}^l$ are $2dfn -fn$, where $\vect{T}\in \mathbb{R}^{n\times f}$ is a temporary matrix. The number of FLOPs for $\vect{\hat{A}}\vect{T}$ are $fm + f(m-n)$, or $2fm - fn$. Plugging $MACs = \frac{FLOPs}{2}$ (same as ULTH for GCN~\cite{chen2021unified}), the total number of MAC operations on $l$-th layer are $\frac{2dfn - fn + 2fm -fn}{2}$, or $(fm+dfn-fn)$.
\end{proof}
\begin{lemma}
\label{lem:lower}
If we introduce $a\%$, $h\%$, and $w\%$ sparsity to $\vect{\hat{A}}$, $\vect{H}^l$, and $\vect{W}^l$, respectively, then the total MAC operations are bounded by $(1-w)(1-h')(fm+dfn-fn)$, where $d > f$ and $a\approx h=h'$.
\end{lemma}
\begin{proof}
For simplicity of the computations, we distribute the percentage of sparsity across matrix dimensions. Then, an $a\%$ sparsity of graph would leave $(1-a)m$ non-zero elements in $\vect{\hat{A}}$, an $h\%$ sparsity of embedding would leave $n\times (1-h)d$ non-zero elements in $\vect{H}$, and a $w\%$ sparsity of weight matrix would leave $(1-h)d\times (1-w)f$ non-zero elements in $\vect{W}$. The right to left order multiplication would cost $(1-h)(1-w)dfn + (1-w)(d-dh-1)fn$ FLOPs for $\vect{T} = \vect{H}^l\vect{W}^l$, where $\vect{T}\in \mathbb{R}^{n\times (1-w)f}$ is a temporary matrix. Similarly, the number of FLOPs for $\vect{\hat{A}}\vect{T}$ are $(1-a)(1-w)fm + (1-a)(1-w)(m-n)f$. Then, the total number of FLOPs on the $l$-th layer are as follows:
\begin{flalign*}
\begin{split}
    & = 2(1-h)(1-w)dfn - (1-w)fn + 2(1-a)(1-w)fm\\ &-(1-a)(1-w)fn\\
   %& = (1-w)\{(1-r)dfn + (1-a)fn^2 + (d-rd-1)fn \\ & + (1-a)(n-1)fn\} \\ 
   & \le 2(1-h)(1-w)dfn + 2(1-a)(1-w)fm -2(1-a)(1-w)fn \\
   & = 2(1-w)\{(1-h)dfn+(1-a)fm-(1-a)fn\} \\
   & = 2(1-w)(1-h')(fm+dfn-fn)
   \end{split}
\end{flalign*}
From the above computational bound, we can derive that the MACs on the $l$-th layer are bounded by $\frac{2(1-w)(1-h')(fm+dfn-fn)}{2}$, or $(1-w)(1-h')(fm+dfn-fn)$.
\end{proof}

\begin{theorem}
\label{theorem:ratio}
For $a\%$, $h\%$, and $w\%$ sparsity to $\vect{\hat{A}}$, $\vect{H}^l$, and $\vect{W}^l$ matrices, the total reduction factor of MAC operations in GCN is bounded by $\frac{1}{(1-w)(1-h')}$, where $a\approx h=h'$.
\end{theorem}
\begin{proof}
This proof is straightforward. We can infer it by taking the ratio of the result of Lemma \ref{lem:upper} to the result of Lemma \ref{lem:lower} that the reduction factor is bounded by $\frac{1}{(1-w)(1-h')}$.
\end{proof}

\textbf{Complexity.} From Lemma  \ref{lem:lower}, we can deduce that the asymptotic time complexity of the sparse training procedure for a $L$-layered GCN would be $O((1-w)(1-h')(m + fn)fL)$, where $f\approx d$, and $|E|=m$. Similarly, the asymptotic memory complexity would be $O(Lf((1-h')n + (1-w)f) + (1-h')m)$.

==> results.tex <==
\section{Experiments}
\subsection{Experimental Setup}
\textbf{Overview.} The goal of our experiments is to explore the sparsity of different matrices in Eqn. \ref{eqn:gcn} without sacrificing the baseline accuracy. 
Considering the limited previous work on the use of combined sparsity in GNNs,
%Though the study of combined sparsity in GNNs is rare in the literature, 
we compare the effectiveness of our sparsification strategies with the work by Chen et al. \cite{chen2021unified}. In our experiments, we aim to address the following Research Questions (RQs). 
\begin{itemize}
    \item \textbf{RQ1:} Which embedding dimensions work the best to induce sparsity in the embedding matrix? 
    %would be the better dimension for embedding matrix to introduce different percentages of sparsity?
    %\item \textbf{RQ2:} How does the sparsity level change with the changes of embedding dimension?

    \item \textbf{RQ2:} How does the performance of node classification vary with individual sparsity techniques?
    
    \item \textbf{RQ3:} Which sparsification technique is better to introduce sparsity in different matrices of Eqn. \ref{eqn:gcn}?
    %\item \textbf{RQ4:} What is the degree distribution of weight matrices after sparsification?
    
    \item \textbf{RQ4:} How does the sparsity change for various graphs having different average degrees?
    
    
\end{itemize}

\textbf{Environment.} We conduct all the experiments of SparseGCN on a server equipped with an Intel(R) Xeon(R) CPU E5-2680 v3 @ 2.50GHz, 24 cores, 32KB L1 cache, 256KB L2 cache, 30MB L3 cache, and 256GB RAM.  We run the experiments of ULTH\footnote{\url{https://github.com/VITA-Group/Unified-LTH-GNN/tree/main/NodeClassification}} on an Nvidia Titan RTX (24GB RAM) with the required system configurations. We have implemented the SparseGCN workflow in the PyTorch-Geometric (PyG) framework version 2.0.0 with PyTorch version 1.9.0 \cite{fey2019pyg}. Unless otherwise mentioned, we use a 2-layered GCN model as the underlying GNN model and develop our workflow on top of it. For all experiments, we use default options available in PyG for different hyper-parameters such as learning rate ($0.01$), \emph{relu} activation function, \emph{Adam} optimizer, and \emph{negative log-likelihood} loss function. To evaluate the performance, we use \emph{accuracy} metric.

\begin{table}[!htb]
\centering
\caption{Summary of the Graph Datasets.}
\vspace{-0.25cm}
\label{tab:dataset}
\begin{tabular}{p{1.25cm}|p{0.75cm}|p{0.82cm}|p{0.86cm}|p{1.1cm}|p{1.4cm}} 
\hline
\textbf{Graphs}    & \textbf{Nodes} & \textbf{Edges}   & \textbf{Classes} & \textbf{Features} & \textbf{Avg. Deg.}  \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
Cora      & 2,708 & 10,556  & 7       & 1,433    & 3.89       \\
Citeseer  & 3,327 & 9,104   & 6       & 3,703    & 2.74       \\ 
Pubmed & 19,717  &   88,648   & 3 &   500 &  4.5 \\
Chameleon & 2,277 & 36,101  & 3       & 3,132    & 15.85       \\ 

Squirrel  & 5,201 & 217,073 & 3       & 3148     & 41.74       \\ 

\hline
\end{tabular}
%\vspace{-7pt}
\end{table}
\vspace{-0.25cm}
\textbf{Datasets.}
We report the summary of our datasets in Table \ref{tab:dataset}. Previous studies mostly analyze Cora, Citeseer, and Pubmed datasets \cite{chen2021unified,you2021gebt}. However, these are scale-free homophilic networks that often react similarly to induced sparsity. To explore more on the sparsity, we also use two heterophilic networks (Chameleon and Squirrel) that have higher average degrees \cite{zhu2020beyond}. The rationale for choosing these two datasets is not only to study graphs with high average degrees, but also to evaluate the impact of sparsifications on heterophilic networks.
Other previous studies related to sparse GNNs ignored these two aspects (average degree and heterophily) in their experiments. 
% on sparsifications which is ignored by previous studies. 
The Cora, Citeseer, and Pubmed datasets are available in PyG whereas Chameleon and Squirrel datasets have been collected from FAGCN \cite{fagcn2021} GitHub repository\footnote{https://github.com/bdy9527/FAGCN}. In our experiments, we create the training, validation, and test sets similar to previous studies \cite{kipf2016semi,chen2021unified} i.e., 20 vertices per label in the training set, 500 vertices for validations, and 1000 vertices for testing.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.75\linewidth]{plots/choose_dimensions.pdf}
    \vspace{-0.25cm}
    \caption{Test accuracy of different graphs for various dimensions of hidden representations.}
    \vspace{-0.25cm}
    \label{fig:choose_dimension}
\end{figure}
\subsection{Results and Analysis}
\textbf{Hidden Dimension.} We first analyze the impact of hidden layer dimensions on the test accuracy of GCN. 
%test accuracy of different graphs based on various dimensional hidden representations. 
We report the results in Fig. \ref{fig:choose_dimension}. The rationale behind this set of experiments is to select a dimension for hidden representation for which we get higher accuracy. Fig. \ref{fig:choose_dimension} shows that the accuracy drops significantly  for Cora and Citeseer when the hidden dimension is less than 16. The accuracy of Chameleon and Squirrel graphs is not very sensitive to the hidden dimension. %does not vary that much for various dimensional embeddings. 
Overall, all graphs show a reasonable level of accuracy for 64-dimensional embeddings (see Fig. \ref{fig:accuracy_dimension} for more results). Thus, unless otherwise mentioned, we choose 64 as the embedding dimension for the rest of our experiments to introduce different percentages of sparsity.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.75\linewidth]{plots/lambda.pdf}
    \vspace{-0.25cm}
    \caption{Test accuracy of the various scaling factor for Sensitivity-based pruning of weight matrices in GCN. Sparsity is reported in Table \ref{tab:lambdasparse}.}
    \label{fig:lambda}
\end{figure}
\begin{table*}[!htb]
\centering
\caption{Percentage of sparsity in the weight matrices of the first layer ($\vect{W}^1$) and the second layer ($\vect{W}^2$) of the GCN model for different values of scaling factor $\lambda$ in Sensitivity-based sparsification. Test accuracy is reported in Fig. \ref{fig:lambda}. Gray colored cells represent better combination of percentages for weight matrices preserving baseline accuracy.}
\label{tab:lambdasparse}
\arrayrulecolor{black}
\begin{tabular}{c|cc|cc|cc|c|cc|cc|cc} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-14}
\multirow{2}{*}{$\lambda$} & \multicolumn{2}{c!{\color{black}\vrule}}{Cora} & \multicolumn{2}{c!{\color{black}\vrule}}{Citeseer} & \multicolumn{2}{c!{\color{black}\vrule}}{Pubmed} & \multirow{2}{*}{$\lambda$} & \multicolumn{2}{c!{\color{black}\vrule}}{Cora} & \multicolumn{2}{c!{\color{black}\vrule}}{Citeseer} & \multicolumn{2}{c}{Pubmed}  \\ 
\cline{2-7}\cline{9-14}
                        & $\vect{W}^1$      & $\vect{W}^2$                                   & $\vect{W}^1$      & $\vect{W}^2$                                       & $\vect{W}^1$      & $\vect{W}^2$                                     &                         & $\vect{W}^1$      & $\vect{W}^2$                         & $\vect{W}^1$      & $\vect{W}^2$                             & $\vect{W}^1$      & $\vect{W}^2$                           \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-14}
0.1                     & 33.71\% & 5.58\%                               & 51.09\% & 8.59\%                                   & 25.51\% & 4.17\%                                 & 1                       & 84.29\% & 37.28\%                              & 84.95\% & 40.89\%                                  & 78.99\% & 42.19\%                                 \\ 
%\hline
0.2                     & 45.16\% & 10.49\%                              & 58.49\% & 20.05\%                                  & 33.72\% & 14.06\%                                & 1.1                     & 86.17\% & 55.58\%                              & 86.60\% & 48.18\%                                  & 81.69\% & 54.69\%                                 \\ 
%\hline
0.3                     & 54.12\% & 15.63\%                              & 64.13\% & 28.91\%                                  & 41.79\% & 18.75\%                                & 1.2                     & {\cellcolor[rgb]{0.8,0.8,0.8}}87.78\% & {\cellcolor[rgb]{0.8,0.8,0.8}}76.56\%                              & 88.08\% & 60.68\%                                  & {\cellcolor[rgb]{0.8,0.8,0.8}}83.89\% & {\cellcolor[rgb]{0.8,0.8,0.8}}69.79\%                                 \\ 
%\hline
0.4                     & 61.18\% & 17.86\%                              & 68.65\% & 31.51\%                                  & 49.27\% & 19.79\%                                & 1.3                     & 89.11\% & 93.97\%                              & 89.40\% & 79.95\%                                  & 85.91\% & 87.50\%                                 \\ 
%\hline
0.5                     & 67.02\% & 18.53\%                              & 72.38\% & 32.81\%                                  & 56.34\% & 20.31\%                                & 1.4                     & 90.31\% & 99.11\%                              & {\cellcolor[rgb]{0.8,0.8,0.8}}90.56\% & {\cellcolor[rgb]{0.8,0.8,0.8}}92.45\%                                  & 87.58\% & 95.31\%                                 \\ 
%\hline
0.6                     & 71.82\% & 19.64\%                              & 75.60\% & 33.59\%                                  & 62.43\% & 22.92\%                                & 1.5                     & 91.33\% & 99.78\%                              & 91.57\% & 99.48\%                                  & 88.98\% & 99.48\%                                 \\ 
%\hline
0.7                     & 75.83\% & 21.21\%                              & 78.35\% & 33.59\%                                  & 67.69\% & 24.48\%                                & 1.6                     & 92.22\% & 99.78\%                              & 92.45\% & 99.74\%                                  & 90.13\% & 99.48\%                                 \\ 
%\hline
0.8                     & 79.14\% & 23.66\%                              & 80.82\% & 35.16\%                                  & 72.11\% & 27.60\%                                & 1.7                     & 93.04\% & 99.78\%                              & 93.22\% & 99.74\%                                  & 91.17\% & 99.48\%                                 \\ 
%\hline
0.9                     & 81.87\% & 28.13\%                              & 83.00\% & 36.98\%                                  & 75.86\% & 32.29\%                                & 1.8                     & 93.67\% & 99.78\%                              & 93.90\% & 99.74\%                                  & 91.95\% & 99.48\%                                 \\
\hline
\end{tabular}
\arrayrulecolor{black}
\end{table*}
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/cora_h.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/cora_w.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/cora_a.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/citeseer_h.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/citeseer_w.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/citeseer_a.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/pubmed_h.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/pubmed_w.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/pubmed_a.pdf}
    \vspace{-0.25cm}
    \caption{The test accuracy of homophilic graphs using different percentages of sparsity for the node classification tasks. The top, middle, and bottom panels show different percentages of sparsity for Cora, Citeseer, and Pubmed graphs, respectively. Baseline accuracy is achieved without introducing any sparsity.}
    \vspace{-0.3cm}
    \label{fig:homophily_sparsity}
\end{figure*}

\textbf{Scaling Factor for Sensitivity-based Pruning.} We analyze the effect of the scaling factor $\lambda$ used in the sensitivity-based pruning of weight matrices. We report the results in Fig. \ref{fig:lambda}. We observe that the accuracy drops for most of the graphs when the value of  $\lambda$ goes above 1.2. More specifically, $\lambda=1.2$ would be a better choice to retain accuracy with higher percentages of weight sparsity for Cora, Citeseer, and Pubmed datasets. We also report the layer-wise weight sparsity for this experiment in Table \ref{tab:lambdasparse}. We observe that the first layer introduces more sparsity to the weight than the second layer for $\lambda < 1.3$ and test accuracy is also retrained as shown in Fig. \ref{fig:lambda}. When $\lambda \ge 1.3$, the weight sparsity of the second layer becomes higher than the first layer and test accuracy drops for Cora and Pubmed. Test accuracy also drops for Citeseer when the weight sparsity of the second layer is comparatively higher than the first layer ($\lambda \ge 1.5$). 
Note that the number of non-zero entries in the weight of the first layer ($\vect{W}^1$) is higher than the number of non-zero entries in the weight of the second layer ($\vect{W}^2$) for all these graphs. Thus, a higher sparsity in the $\vect{W}^1$ matrix is desirable. 
%The best choice of $\lambda$ automatically s 
Interestingly enough, this sensible choice of unequal weight sparsity is automatically coming from $\lambda$.

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/chameleon_h.pdf}
    \includegraphics[width=0.32\linewidth,height=3.2cm]{plots/chameleon_w.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/chameleon_a.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/squirrel_h.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/squirrel_w.pdf}
    \includegraphics[width=0.32\linewidth,height=3.3cm]{plots/squirrel_a.pdf}
    \vspace{-0.25cm}
    \caption{The sparsity of heterophilic graphs for the node classification task. The top and bottom panels show different levels of sparsity for Chameleon, and Squirrel graphs, respectively. Baseline accuracy is achieved without introducing any sparsity.}
    \label{fig:heterophily_sparsity}
\end{figure*}
\textbf{The Sparsity of Low-average Degree Graphs.} We report the sparsity of different low-average degree homophilic graphs in Fig. \ref{fig:homophily_sparsity}. Here, we show the test accuracy for three different sparsification techniques, namely, (i) Random, (ii) Top-$k$, and (iii) Sorting-based. Notice that the $x$-axis represents different specific percentages of sparsity. We exclude the results for the Sensitivity-based technique since we can not specify the percentage of sparsity in this approach.

\begin{observation}
\label{obs:embedding}
The Top-$k$ approach can retain the baseline accuracy with a higher percentage of sparsity in the embedding matrix than other sparsification techniques.
\end{observation}
In the sparsity results of embedding matrix (see Fig. ~\ref{fig:homophily_sparsity}, left column), we observe that the Top-$k$ method can retain the baseline accuracy level with a higher percentage of sparsity compared to the random and sorting-based techniques. The Top-$k$ approach is a local sparsification technique that prunes the same number of entries from each row of the embedding matrix based on the absolute value. The impact of the top-k pruning is similar to reducing the hidden dimension to $k$ (assuming that $k$ is indeed smaller than the hidden dimension). %This is similar to reducing the dimensions of the embedding pruning insignificant entries. 
% \checkme{
% Thus, we observe a similar range of accuracy even with 50\% sparsity. We can compare the accuracy of Cora, Citeseer, and Pubmed with respect to the accuracy of 32-dimensional embedding in Fig. \ref{fig:choose_dimension}. We observe that they are similar or differ by a tiny amount.} 
The random strategy performs the  worst among all methods. The random technique is similar to adding \emph{dropout} to the neural network for regularization, but it does not retain accuracy as seen in Fig. ~\ref{fig:homophily_sparsity}.
%the Top-$k$ approach might serve the purpose better with on-the-fly regularization. this is an unproven comment that we should avoid. 
\begin{observation}
\label{obs:weight}
The Sorting-based approach can retain the baseline accuracy with a higher percentage of sparsity in the weight matrix and adjacency matrix than the other sparsification techniques.
\end{observation}
In the experiments of neural network weight sparsity (see Fig. \ref{fig:homophily_sparsity}, middle column), we add the same percentage of sparsity to both layers of the GCN. We observe results similar to previous studies, which suggests that the sorting-based method can retain the baseline accuracy better than others with a higher percentage of sparsity \cite{chen2021unified}. Notice that the Top-$k$ method can be competitive to the Sorting-based method. For Cora, Citeseer, and Pubmed networks in Fig. \ref{fig:homophily_sparsity}, we observe that the Sorting-based approach can achieve a better level of graph sparsity. The average degree of Cora and Citeseer is comparatively low i.e., they are already very sparse. Making these graphs sparser may disconnect some vertices, which prevents information propagation from neighbors. Thus, even with a small percentage of sparsity in Cora and Citeseer, test accuracy tends to drop. On the other hand, the Pubmed graph is comparatively bigger. Thus, pruning some edges does not affect the test accuracy significantly. For example, the Sorting-based approach can retain the baseline accuracy with up to 40\% graph sparsity, whereas test accuracy drops above 20\% graph sparsity for Cora and Citeseer.  

From the experimental results of Fig. \ref{fig:homophily_sparsity}, we observe that the homophilic graphs are more sensitive to the graph sparsity than the neural network weight. In other words, the baseline accuracy cannot be preserved by introducing the same maximum possible percentage of sparsity to all matrices in Eqn. \ref{eqn:gcn}.  


\textbf{The Sparsity of High-average Degree Graphs.} We report the sparsity results for comparatively high-average degree graphs in Fig. \ref{fig:heterophily_sparsity}. For embedding sparsity, we observe similar results to homophilic graphs as outlined in Observation \ref{obs:embedding} i.e., Top-$k$ approach attains the baseline accuracy with a higher percentage of embedding sparsity. For the weight sparsity, the results are not obvious. However, the Sorting-based technique shows competitive performance to retain baseline accuracy with a higher percentage of sparsity. 
\begin{observation}
\label{obs:graph}
Graphs with a high average degree are less sensitive to graph sparsity than the graphs with a low average degree. 
\end{observation}
In Fig. \ref{fig:heterophily_sparsity}, we observe that the Sorting-based approach can retain the baseline accuracy with a higher percentage of sparsity. This percentage is higher compared to the sparsity of homophilic networks shown in Fig. \ref{fig:homophily_sparsity}. More specifically, the Sorting-based method can attain the baseline accuracy with 90\% graph sparsity for the Squirrel dataset whereas, this percentage of sparsity for homophilic low average degree graphs is only up to 40\% (Pubmed graph). Notice that the average degree of the Squirrel graph is around 42, which is almost seven times higher than the average degree of the Pubmed graph. Thus, the average degree plays an important role in the analysis of graph sparsity. The rationale is that graphs with a high average degree offer more edges to prune than the graphs with a low average degree. 
% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}[!htb]
\centering
\caption{Weight sparsity of GCN model for homophilic graphs using Sorting and Sensitivity-based techniques. The compression ratio is computed by dividing the number of parameters in the original GCN model by the number of parameters in a sparse model.}
\label{tab:compression}
\arrayrulecolor{black}
\begin{tabular}{c|c|cc|cc} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
\multirow{2}{*}{Graphs} & \multirow{2}{*}{GCN Model} & \multicolumn{2}{c!{\color{black}\vrule}}{\#Sparse Parameters} & \multicolumn{2}{c}{Compress. Ratio}  \\ 
\cline{3-6}
                        &                        \#parameters    & Sort & Sense                                        & Sort & Sense                                        \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
Cora                    & 92,160                      & 13,825   & {\cellcolor[rgb]{0.851,0.918,0.827}}11,310                                              & 6.67    & {\cellcolor[rgb]{0.851,0.918,0.827}}8.15                                               \\ 
%\hline
Citeseer                & 237,376                     & 23,739   & {\cellcolor[rgb]{0.851,0.918,0.827}}22,400                                              & 10.00   & {\cellcolor[rgb]{0.851,0.918,0.827}}10.60                                              \\ 
%\hline
Pubmed                  & 32,192                      & {\cellcolor[rgb]{0.851,0.918,0.827}}3,220    & 5,213                                               & {\cellcolor[rgb]{0.851,0.918,0.827}}10.00   & 6.18                                               \\
\hline
\end{tabular}
\arrayrulecolor{black}
\end{table}

\textbf{Compression ratio of GCN model for Homophilic Graphs.} The weight parameters of a GNN model contribute to a significant part of the training or inference time, especially with the deeper models \cite{li2021training}. Thus, being able to compress or reduce the number of model parameters without sacrificing  the baseline accuracy is desirable to speed up the computations of neural networks \cite{chen2021unified,choudhary2020comprehensive,deng2020model}. In this paper, we analyze the compression ratio of the GCN model empirically employing Sorting-based and Sensitivity-based sparsification techniques. We summarize the results for homophilic graphs in Table \ref{tab:compression} where all techniques retain the baseline test accuracy. For Sensitivity-based pruning, we set $\lambda=1.2$ for Cora and Pubmed graphs, and $\lambda=1.4$ for the Citeseer graph. In Table \ref{tab:compression}, we can see that the Sensitivity-based pruning achieves a better compression ratio (up to 10.6$\times$) for Cora and Citeseer graphs whereas the Sorting-based method achieves a better compression ratio for the Pubmed graph.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.46\linewidth,height=2.3cm]{plots/cora_degree_before.pdf}
    \includegraphics[width=0.5\linewidth,height=2.3cm]{plots/cora_degree_after.pdf}
    \caption{Degree distribution of Cora graph before (left plot), and after introducing sparsity (right plot) using Sorting-based technique.}
    \vspace{-0.25cm}
    \label{fig:degree_cora}
\end{figure}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.54\linewidth,height=2.3cm]{plots/squirrel_degree_before.pdf}
    \includegraphics[width=0.43\linewidth,height=2.3cm]{plots/squirrel_degree_after.pdf}
    \caption{Degree distribution of Squirrel graph before (left plot), and after introducing sparsity (right plot) using Sorting-based technique.}
    \label{fig:degree_squirrel}
\end{figure}

\textbf{Degree Distributions of Sparsified Graphs.} We analyze the degree distribution of graphs before and after introducing the sparsity. We observe that both homophilic and heterophilic networks show similar types of results. 
\begin{observation}
\label{obs:graph_sparsity}
The Sorting-based sparsification technique prunes edge(s) from the high-degree vertices of the graph.  
\end{observation}
We show the degree distribution of Cora and Squirrel graphs in Figs. \ref{fig:degree_cora}, and \ref{fig:degree_squirrel}. The percentage of sparsity for Cora and Squirrel graphs are 20\%, and 90\% respectively. The highest degree of a vertex for the Cora graph is above 150 whereas, it drops below 50 after the sorting-based sparsification. For the squirrel graph, the high average degree drops from 264 to 71. Since the Sorting-based approach prunes edge based on the edge weight, high degree vertices tend to have low edge weight due to the normalization. As a result, the incident edges of the high degree vertices are mostly selected for pruning. We also observe similar results for other graphs (e.g., Chameleon in Fig. \ref{fig:degree_chameleon}).

% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}[!htb]
\centering
\caption{Comparison of combined sparsity and test accuracy between ULTH and SparseGCN. The sparsity in each row of columns $\vect{\hat{A}}$, $\vect{W}$, and $\vect{H}$, are used combinedly.}
\label{tab:comparison}
\arrayrulecolor{black}
\begin{tabular}{c|c|ccc|c} 
\hline
\textbf{Graphs}                    & \textbf{Methods}   & \textbf{$\vect{\hat{A}}$}                                 & \textbf{$\vect{W}$}                                 & \textbf{$\vect{H}$} & \textbf{Accuracy}                                    \\ \hline

\multirow{2}{*}{Cora}     & ULTH~\cite{chen2021unified}      & 14.8\%                                     & 59.1\%                                     & 0.0\%      & 80.0\%                                      \\ 

                          & SparseGCN & 14.5\%                                     & 61.0\%                                     & {\cellcolor[rgb]{0.851,0.918,0.827}}8.4\%      & 80.0\%                                      \\ 
\hline
\multirow{2}{*}{Citeseer} & ULTH~\cite{chen2021unified}       & 19.0\%                                     & 70.1\%                                     & 0.0\%      & 71.5\%                                      \\ 

                          & SparseGCN & 19.1\%                                     & 70.8\%                                     & {\cellcolor[rgb]{0.851,0.918,0.827}}9.8\%      & 71.4\%                                      \\ 
\hline
\multirow{2}{*}{Pubmed}   & ULTH~\cite{chen2021unified}       &  20.6\% & 70.0\% & 0.0\%      &  77.8\% \\ 

                          & SparseGCN & 23.0\%                                     & 75.0\%                                     & {\cellcolor[rgb]{0.851,0.918,0.827}}11.5\%     & 80.0\%                                      \\
\hline
\end{tabular}
\arrayrulecolor{black}
\end{table}

\textbf{Comparison with Unified Lotter Ticket Hypothesis.}
We compare our results with ULTH~\cite{chen2021unified} which is a state-of-the-art approach to introduce sparsity to the adjacency matrix and model weights in GNNs. To introduce sparsity using SparseGCN, we use the Top-$k$ approach for the embedding matrix, $\vect{H}$ (Observation \ref{obs:embedding}) and the Sorting-based approach for other matrices. We run both ULTH and SparseGCN for 64-dimensional embedding and report the results in Table \ref{tab:comparison} (see Fig. \ref{fig:compare_weight_ulth} for more comparisons). We use a grid search technique to find the highest possible sparsity in different matrices retaining a similar level of test accuracy compared to the baseline. We observe that both ULTH and SparseGCN attain a similar level of test accuracy with similar percentages of sparsity in $\vect{\hat{A}}$, and $\vect{W}$; however, SparseGCN introduces additional sparsity to the embedding matrix. More specifically, SparseGCN can introduce 8.4\% and 9.8\% more sparsity to the embedding matrix for the Cora and Citeseer dataset with a similar level of test accuracy. For the Pubmed graph, the level of sparsity, as well as test accuracy, outperform ULTH. These empirical results show the effectiveness of employing SparseGCN to introduce sparsity in different matrices of GCN. 


==> summplementary.tex <==
%\onecolumn
\begin{table*}[!htb]
    \centering
    \begin{tabular}{c}
     \textbf{\huge{Supplementary Figures}}
    \end{tabular}
\end{table*}
\begin{figure*}[p]
    \centering
    \includegraphics[width=0.35\linewidth,height=3.2cm]{plots/chameleon_degree_before.pdf}
    \includegraphics[width=0.35\linewidth,height=3.2cm]{plots/chameleon_degree_after.pdf}
    \caption{(Supplement) Degree distribution of Chameleon graph before sparsification (left plot), and after sparsification (right plot) employing Sorting-base technique. We introduce 50\% graph sparsity for this graph which is derived from the Fig. \ref{fig:heterophily_sparsity}.}
    \label{fig:degree_chameleon}
\end{figure*}

\begin{figure*}[!htb]
    \centering
    \begin{subfigure}{.40\linewidth}
  \centering
  \includegraphics[width=0.99\linewidth,height=4.cm]{plots/cora_topk_dim.pdf}
  \caption{Cora graph}
    \label{fig:cora_topk_dim}
\end{subfigure}
\begin{subfigure}{.4\linewidth}
  \centering
   \includegraphics[width=0.99\linewidth,height=4.cm]{plots/chameleon_topk_dim.pdf}
   \caption{Chameleon graph}
    \label{fig:chameleon_topk_dim}
\end{subfigure}
    \caption{(Supplement) Test accuracy of (a) Cora, and (b) Chameleon graphs introducing the sparsity on various dimensional embedding using Top-$k$ approach. Cora graph shows similar performance for different dimensional embeddings up to 55\% emedding sparsity whereas Chameleon graph shows better accuracy for 64-dimensional embedding.}
    \label{fig:accuracy_dimension}
\end{figure*}



\begin{figure*}[!htb]
    \centering
    \begin{subfigure}{.32\linewidth}
  \centering
  \includegraphics[width=0.99\linewidth,height=2.3cm]{plots/cora_weight_distribution_W1.pdf}
  \caption{for $W_1$ of Cora}
  %\caption{Layer-wise validation accuracy in GCN model for Cora network.}
  \label{fig:layers_contribution}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
  \centering
   \includegraphics[width=0.99\linewidth,height=2.3cm]{plots/citeseer_weight_distribution.pdf}
   \caption{for $W_1$ of Citeseer}
  %\caption{Comparison among multi-layered GNNs for Email network.}
  \label{fig:multiple_layers}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
  \centering
   \includegraphics[width=0.99\linewidth,height=2.3cm]{plots/pubmed_weight_distribution.pdf}
   \caption{for $W_1$ of Pubmed}
  %\caption{Comparison among multi-layered GNNs for Email network.}
  \label{fig:multiple_layers}
\end{subfigure}

    \caption{(Supplement) Distribution of the number of non-zeros in the first layer weight matrix $W_1$ with respect to the number of rows after introducing Sorting-based sparsification for (a) Cora, (b) Citeseer, and (c) Pubmed graphs (weight sparsity = 85\%).}
    \label{fig:weight_degree}
\end{figure*}


\begin{figure*}[!htb]
    \centering
    \begin{subfigure}{.32\linewidth}
  \centering
  \includegraphics[width=0.99\linewidth,height=2.5cm]{plots/compare_cora_w_ulth.pdf}
  \caption{Weight Sparsity for Cora}
  %\caption{Layer-wise validation accuracy in GCN model for Cora network.}
  \label{fig:compare_cora}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
  \centering
   \includegraphics[width=0.99\linewidth,height=2.5cm]{plots/compare_citeseer_w_ulth.pdf}
   \caption{Weight Sparsity for Citeseer}
  %\caption{Comparison among multi-layered GNNs for Email network.}
  \label{fig:compare_citeseer}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
  \centering
   \includegraphics[width=0.99\linewidth,height=2.5cm]{plots/compare_pubmed_w_ulth.pdf}
   \caption{Weight Sparsity for Pubmed}
  %\caption{Comparison among multi-layered GNNs for Email network.}
  \label{fig:compare_pubmed}
\end{subfigure}

    \caption{(Supplement) Comparison of weight sparsity among SparseGCN (Sorting-based technique) and ULTH~\cite{chen2021unified} with respect to the baseline accuracy using (a) Cora, (b) Citeseer, and (c) Pubmed graphs.}
    \label{fig:compare_weight_ulth}
\end{figure*}
%https://towardsdatascience.com/sparse-matrices-in-pytorch-be8ecaccae6





